Exact Support Recovery for Sparse Spikes Deconvolution

This paper studies sparse spikes deconvolution over the space of measures. We focus our attention to the recovery properties of the support of the measure, i.e. the location of the Dirac masses. For non-degenerate sums of Diracs, we show that, when the signal-to-noise ratio is large enough, total variation regularization (which is the natural extension of the L1 norm of vectors to the setting of measures) recovers the exact same number of Diracs. We also show that both the locations and the heights of these Diracs converge toward those of the input measure when the noise drops to zero. The exact speed of convergence is governed by a specific dual certificate, which can be computed by solving a linear system. We draw connections between the support of the recovered measure on a continuous domain and on a discretized grid. We show that when the signal-to-noise level is large enough, the solution of the discretized problem is supported on pairs of Diracs which are neighbors of the Diracs of the input measure. This gives a precise description of the convergence of the solution of the discretized problem toward the solution of the continuous grid-free problem, as the grid size tends to zero.

==> sections/sec-ideal-lowpass.tex <==
% !TEX root = ../DuvalPeyre-SparseSpikes.tex

\section{Application to the Ideal Low-pass Filter}
\label{sec-idealLP}

In this section, we apply the results of the previous sections to the particular case of the Dirichlet kernel, defined as
\begin{align}
	\varphi(t) = \sum_{k=-f_c}^{f_c} e^{2i\pi kt} = \frac{\sin \left((2f_c+1)\pi t\right)}{\sin (\pi t)}.
\end{align}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Elementary Results}

We first check that the assumptions made in Section~\ref{sec-noise-robust} hold in the case of the ideal low-pass filter.


\begin{prop}[Existence of $p_0$]
Let $m\in \Mm(\TT)$ and $y=\Phi m\in L^2(\TT)$. There exists a solution of~\eqref{eq-constrained-dual}.
As a consequence, $p_0\in L^2(\TT)$ is well defined.
\end{prop}

\begin{proof}
We rewrite~\eqref{eq-constrained-dual} as 
\eq{
	\usup{\normi{\eta} \leq 1, \eta \in \Im \Phi^*} \dotp{m}{\eta}.
}
Let $(\eta_n)_{n\in \NN}$ be any maximizing sequence. Then $(\eta_n)_{n\in \NN}$ is bounded in the finite-dimensional space of trigonometric polynomials with degree $f_c$ or less. We may extract a subsequence converging to $\eta^*\in C(\TT)$. But $\normi{\eta^*} \leq 1$ and $\eta^*\in \Im \Phi^*$,
so that $\eta^*=\Phi^*p^*$ for some $p^*$ solution of~\eqref{eq-constrained-dual}.
\end{proof}

\begin{prop}[Injectivity of $\Ga_{x}$]
Let $x=(x_1,\ldots x_N)\in \TT^N$ with $x_i\neq x_j$ for $i\neq j$ and $N\leq f_c$.
Then $\Ga_x=(\Phi_x, \Phi_x')$ has full rank.
\end{prop}

\begin{proof}
Assume that for some $(u,v)\in \RR^N\times \RR^N$, $\Ga_x (u,v)=0$. Then
\begin{align*}
	\foralls  t\in \TT, \quad 0&=\sum_{j=1}^N  \left(u_j\varphi(t-x_j)+v_j \varphi'(t-x_j)\right)\\
&=\sum_{k=-f_c}^{f_c} \left(\sum_{j=1}^N (u_j + 2ik\pi v_j)e^{-2ik\pi x_j}  \right) e^{2ik\pi t}
\end{align*}
We deduce that 
\eq{
	\foralls k\in \{-f_c,\ldots f_c \}, \quad
	\sum_{j=1}^N (u_j + k \tilde{v}_j)r_j^k =0
	\qwhereq
	\choice{
		r_j=e^{-2i\pi x_j},\\
		\tilde{v}_j=2i\pi v_j.
	}
}
It is therefore sufficient to prove that the columns of the following matrix are linearly independent
\begin{align*}
\begin{pmatrix}
r_1^{-f_c} & \ldots &r_N^{-f_c} & (-f_c)r_1^{-f_c}& \ldots &(-f_c)r_N^{-f_c} \\
\vdots & &\vdots  & \vdots & &\vdots \\
r_1^{k} & \ldots &r_N^{k} & kr_1^{k}& \ldots &k r_N^{k} \\
\vdots & &\vdots  & \vdots & &\vdots \\
r_1^{f_c} & \ldots &r_N^{f_c} & (f_c)r_1^{f_c}& \ldots &(f_c)r_N^{f_c} \\
\end{pmatrix}.
\end{align*}
% Since we have not found this result in standard textbooks, we detail the argument.
If $N<f_c$, we complete the family $\{r_1, \ldots r_N\}$ in a family $\{r_0,r_1,\ldots r_{f_c}\}\subset \SS^1$ such
 that the $r_i$'s are pairwise distinct. We obtain a square matrix $M$ by inserting the corresponding columns
\begin{align*}
M = \begin{pmatrix}
r_1^{-f_c} & \ldots &r_{f_c}^{-f_c} & r_0^{-f_c} &(-f_c)r_1^{-f_c}& \ldots &(-f_c)r_{f_c}^{-f_c} \\
\vdots & &\vdots  &\vdots & \vdots & &\vdots \\
r_1^{k} & \ldots &r_{f_c}^{k} & r_0^k &kr_1^{k}& \ldots &k r_{f_c}^{k} \\
\vdots & &\vdots &\vdots & \vdots & &\vdots \\
r_1^{f_c} & \ldots &r_{f_c}^{f_c} & r_0^{f_c}&(f_c)r_1^{f_c}& \ldots &(f_c)r_{f_c}^{f_c} \\
\end{pmatrix}.
\end{align*}
 We claim that $M$ is invertible. Indeed, if there exists $\alpha\in \CC^{(2f_c+1)}$ such that
  $M^T \alpha=0$, then the rational function $F(z) = \sum_{k=-f_c}^{f_c} \alpha_k z^{k}$ satisfies:
\begin{align*}
  	F(r_j)&=0 \qandq F'(r_j)=0 \ \mbox{ for } 1\leq j \leq f_c,\\
  	F(r_0)&=0.
\end{align*}
Hence, $F$ has at least $2f_c+1$ roots in $\SS^1$, counting the multiplicities. This imposes that $F=0$, thus $\alpha=0$,
 and $M$ is invertible. The result is proved.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Identifiable Measures}

In~\cite{Candes-toward}, Cand\`es and Fernandez-Granda have proved that discrete
 measures are identifiable provided that their support is separated enough, i.e. $\Delta(m) \geq \frac{C}{f_c}$ for some $C>0$, where $\Delta(m)$ is the so-called minimum separation distance.

\begin{defn}[Minimum separation]
The minimum separation of the support of a discrete measure $m$ is defined as
\eq{
 	\Delta(m)=\inf_{(t,t')\in \supp (m)} |t-t'|,
}
where $|t-t'|$ is the distance on the torus between $t$ and $t'\in \TT$, and we assume $t\neq t'$.
\end{defn}

In~\cite{Candes-toward} it is proved that $C \leq 2$ for complex measures (i.e. of the form $m_{a,x}$ for $a \in \CC^N$ and $x \in \TT^N$) and $C \leq 1.87$ for real measures (i.e. of the form $m_{a,x}$ for $a \in \RR^N$ and $x \in \TT^N$). Extrapolating from numerical simulations on a finite grid, the authors conjecture that for complex measures, one has $C\geq 1$. In this section we show that for real measures, necessarily $C\geq \frac{1}{2}$.


% Since real measures seem easier to reconstruct than complex measures, and this conjecture being based on building adversarial complex signals, a smaller constant $C$ might be sufficient for real measures. In this section, we prove that for real measures, we must have $C\geq \frac{1}{2}$.

We rely on the following theorem, proved by P. Tur\'an~\cite{Turan1946}.

\begin{thm}[Tur\'an]
Let $P(z)$ be a non trivial polynomial of degree $n$ such that $|P(1)|=\max_{|z|=1} |P(z)|$. Then for any root $z_0$ of $P$ on the unit circle, $|\arg (z_0)|\geq \frac{2\pi}{n}$. Moreover, if $|\arg (z_0)|= \frac{2\pi}{n}$, then $P(z)=c(1+z)^n$ for some $c\in \CC^*$.
 \label{thm-turan}
\end{thm}

From this theorem we derive necessary conditions for measure that can be reconstructed by~\eqref{eq-constrained-pbm}.

\begin{cor}[Non identifiable measures]
Let $\theta\in (0,\frac{1}{2}]$. Then there exists a discrete measure $m$ with $\Delta(m)=\frac{\theta}{f_c}$ such that $m$ is not a solution of~\eqref{eq-constrained-pbm} for $y=\Phi m$.
\end{cor}

\begin{proof}
Let $m=\delta_{-\theta/f_c}+\delta_{0} - \delta_{\theta/f_c}$. By contradiction, assume that $m$ is a solution to ~\eqref{eq-constrained-pbm},
 and let $\eta\in C(\TT)$ be an associated solution of~\eqref{eq-constrained-dual} (which
  exists since $\Im \Phi^*$ is finite-dimensional).
Then necessarily $\eta(0)=1$ and $\eta(\theta/f_c)=-1$.
The real trigonometric polynomial $D(t)=\frac{1+\eta(t)}{2}$ is non-negative,
 $D(0)=1=\normi{D}$ and $D(\theta/f_c)=0$. If $D(t)=\sum_{k=-f_c}^{f_c}d_k e^{2i\pi kt}$,
  the polynomial $P(z) = \sum_{k=0}^{2f_c}d_{k-f_c}z^k$ satisfies $P(1)=1=\sup_{|z|=1}|P(z)|$,
   and $P(e^{2i\pi\frac{\theta}{f_c}})=0$.
   
If $\theta<\frac{1}{2}$ this contradicts Theorem~\ref{thm-turan}. If $\theta=\frac{1}{2}$,
 then Theorem~\ref{thm-turan} asserts that $P(z)=c(1+z)^{2f_c}$, and from $P(1)=1$ we get $c=\frac{1}{2^{2f_c}}$,
 so that 
 \begin{align*}
 D(t)=e^{-2i\pi f_c}P(e^{2i\pi t})=\left(\cos (\pi f_c t)\right)^{2f_c}.
 \end{align*}
 Then $D(-\frac{\theta}{f_c})=0$, which contradicts the optimality of $\eta$.
As a conclusion, $m$ is not a solution of~\eqref{eq-constrained-pbm}. 
\end{proof}

In a similar way, we may also deduce the following corollary.

\begin{cor}
Let $\tilde{m}_\la=m_{\tilde{a}_\la,\tilde{x}_\la}$ be a discrete solution of Problem $\Pp_\la(y+w)$ where $y=\Phi m$ for any data $m\in \Mm(\TT)$ and any noise $w\in L^2(\TT)$. Let $(\tilde{x}_{\la,i}, \tilde{x}_{\la,j}) \in \supp (m_\la)^2$. If $|\tilde{x}_{\la,i}-\tilde{x}_{\la,j}|\leq \frac{0.5}{f_c}$
then $\sign (\tilde{a}_{\la,j})=\sign (\tilde{a}_{\la,i})$.
\end{cor}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Performance of Pre-certificates}

In order to prove their identifiability result for measures, the authors of~\cite{Candes-toward} introduce a ``good candidate'' for a dual certificate associate to $m=m_{a,x}$ for $a \in \CC^N$ and $x \in \RR^N$. 
For $K$ being the square of the Fejer kernel, they build a trigonometric polynomial
\eq{
	\hat \eta_0(t)=\sum_{i=1}^N \left(\alpha_{i}K(t-x_i) + \beta_{i}K'(t-x_i) \right) \mbox{ with } K(t)=\left(\frac{\sin \left(\left(\frac{f_c}{2}+1 \right)\pi t\right)}{\left(\frac{f_c}{2}+1\right)\sin \pi t}\right)^4
}
and compute $(\al_i,\be_i)_{i=1}^N$ by imposing that $\hat \eta_0(x_i)=\sign (a_i)$ and $\hat \eta_0'(x_i)=0$.

They show that the constructed ``pre-certificate'' is indeed a certificate,  i.e. that $\normi{\hat \eta} \leq 1$, provided that the support is separated enough (i.e. when $\Delta(m)\geq C/f_c$). This results is important since it proves that measures that have sufficiently separated spikes are identifiable. Furthermore, using the fact that $\hat \eta_0$ is not degenerate (i.e. $\hat \eta_0(x_i)'' \neq 0$ for all $i=1,\ldots,N$), the same authors derive  an $L^2$ robustness to noise result in~\cite{Candes-superresol-noisy}, and Fernandez-Granda and Azais et al.  use the constructed certificate to analyze finely the positions of the spikes in~\cite{Fernandez-Granda-support,Azais-inaccurate}.
  
  


From a numerical perspective, we have investigated how this pre-certificate compares with the vanishing derivative pre-certificate that appears naturally in our analysis, by generating random real-valued measures for different separation distances and observing  when each pre-certificate satisfies $\normi{\eta} \leq 1$.


\begin{figure}[ht]
\centering
	\begin{tabular}{@{}c@{\hspace{1mm}}c@{}}
	   \includegraphics[width=0.46\linewidth] {precertif-2p5.pdf} &
   		\includegraphics[width=0.46\linewidth] {precertif-1p26.pdf} \\
		$\Delta(m)\approx 2.50/f_c$ & $\Delta(m)\approx 1.26/f_c$ \\[3mm]
	   \includegraphics[width=0.46\linewidth] {precertif-0p69.pdf} &
	   \includegraphics[width=0.46\linewidth] {precertif-0p44.pdf}\\
		$\Delta(m)\approx 0.69/f_c$ & $\Delta(m)\approx 0.44/f_c$
	\end{tabular}
\caption{\label{fig-precertif} % 
The blue curve is the square Fejer kernel pre-certificate $\hat \eta_0$ (introduced in~\cite{Candes-toward}) and the green curve shows the vanishing derivative pre-certificate $\bar\eta_0$, defined in~\eqref{eq-vanishing-der-certif}, for several measures $m$ (whose Diracs' locations and elevation are display in dashed red) with different separation distances $\De(m)$. Eventually when $\Delta(m)$ is small enough, both pre-certificates break (i.e. are not anymore certificates), but the square Fejer always breaks before the vanishing derivative pre-certificate.\vspace{2mm}}
\end{figure}

As predicted by the result of~\cite{Candes-toward}, we observe numerically that the pre-certificate $\hat \eta_0$ is a a certificate (i.e. $\normi{\hat \eta_0} \leq 1$) for any measure with $\De(m) \geq 1.87/f_c$. We also observe that this continues to hold up to $\De(m) \geq 1/f_c$. Yet, below $1/f_c$, we observe numerically that some measures are still identifiable (as asserted using the vanishing derivative pre-certificate $\bar \eta_0$)  but $\hat \eta_0$ stops being a certificate, i.e. $\normi{\hat \eta_0} > 1$. An illustration is given in Figure~\ref{fig-precertif}, where the chosen parameters are $f_c=26$ and $N=7$. For the cases $\Delta(m)=2.50/f_c$ and $\Delta(m)=1.26/f_c$, both pre-certificates $\bar\eta_0$ and $\hat\eta_0$ are certificates, showing that the generated measure is identifiable. Notice how the vanishing derivative certificate $\bar\eta_0$ oscillates much more than the square Fejer certificate $\hat\eta_0$ . For $\Delta(m)=0.69/f_c$, the square Fejer pre-certificate breaks the constraint ($\normi{\eta} \approx 2.39$) whereas the vanishing derivative certificate still satisfies $\normi{\eta} \leq 1$. Eventually, for $\Delta(m)=0.44/f_c$, both pre-certificates violate the constraint, with $\normi{\hat\eta_0} \approx 3.39$ and $\normi{\bar\eta_0}=1.17$ respectively. 
 

In all the experiments that we have led, the vanishing derivative pre-certificate behaved at least as well as the square Fejer. We are not able to prove rigorously this observation, but several facts advocate for this:
\begin{itemize}
 	\item Whenever the square Fejer pre-certificate works, $m$ is a solution of~\eqref{eq-constrained-pbm}, and the minimal norm certificate $\eta_0$
 is then associated to $m$.
 
 	\item Provided that  $|\eta_0| <1$ on $\TT\setminus \supp (m)$ and that $\eta_0''(x_i)\neq 0$
  for all $1\leq i\leq N$, Proposition~\ref{prop-vanish-certif} implies that the
   vanishing derivative pre-certificate $\bar\eta_0$ is equal to $\eta_0$.

	\item It the minimum separation condition holds, the authors of~\cite{Candes-toward} have proved that 
$|\hat \eta_0| <1$ on $\TT\setminus \supp (m)$ and $\hat \eta_0''(x_i)\neq 0$.
\end{itemize}
Intuitively it seems very unlikely that the minimal norm certificate should fail to satisfy $|\eta_0| <1$ on $\TT\setminus \supp (m)$ and $\eta_0''(x_i)\neq 0$ whereas the  square Fejer certificate does not. Indeed the failure of any of those conditions tend to impose a large $L^2$ norm on the considered pre-certificate $\eta$ (recall that when $\phi$ is an ideal low pass filter $\norm{\eta}_2=\norm{p}_2$).
 
 
 
 
